A 3-3-1 model with right-handed neutrinos based on the $\Delta\left(27\right)$ family symmetry

We present the first multiscalar singlet extension of the 3-3-1 model with right-handed neutrinos, based on the $\Delta \left( 27\right) $ family symmetry, supplemented by the $Z_{4}\otimes Z_{8}\otimes Z_{14}$ flavor group, consistent with current low energy fermion flavor data. In the model under consideration, the light active neutrino masses are generated from a double seesaw mechanism and the observed pattern of charged fermion masses and quark mixing angles is caused by the breaking of the $\Delta \left( 27\right) \otimes Z_{4}\otimes Z_{8}\otimes Z_{14}$ discrete group at very high energy. Our model has only 14 effective free parameters, which are fitted to reproduce the experimental values of the 18 physical observables in the quark and lepton sectors. The obtained physical observables for the quark sector agree with their experimental values, whereas those ones for the lepton sector also do, only for the inverted neutrino mass hierarchy. The normal neutrino mass hierarchy scenario of the model is disfavored by the neutrino oscillation experimental data. We find an effective Majorana neutrino mass parameter of neutrinoless double beta decay of $m_{\beta \beta }=$ 22 meV, a leptonic Dirac CP violating phase of $34^{\circ }$ and a Jarlskog invariant of about $10^{-2}$ for the inverted neutrino mass spectrum.

==> biblio5.tex <==
%\cite{Aad:2012tfa}
\bibitem{Aad:2012tfa} 
  G.~Aad {\it et al.} [ATLAS Collaboration],
  %``Observation of a new particle in the search for the Standard Model Higgs boson with the ATLAS detector at the LHC,''
  Phys.\ Lett.\ B {\bf 716}, 1 (2012)
  doi:10.1016/j.physletb.2012.08.020
  [arXiv:1207.7214 [hep-ex]].
  %%CITATION = doi:10.1016/j.physletb.2012.08.020;%%
  %5990 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Chatrchyan:2012xdj}
\bibitem{Chatrchyan:2012xdj} 
  S.~Chatrchyan {\it et al.} [CMS Collaboration],
  %``Observation of a new boson at a mass of 125 GeV with the CMS experiment at the LHC,''
  Phys.\ Lett.\ B {\bf 716}, 30 (2012)
  doi:10.1016/j.physletb.2012.08.021
  [arXiv:1207.7235 [hep-ex]].
  %%CITATION = doi:10.1016/j.physletb.2012.08.021;%%
  %5846 citations counted in INSPIRE as of 28 Apr 2016



%\cite{An:2012eh}
\bibitem{An:2012eh} 
  F.~P.~An {\it et al.} [Daya Bay Collaboration],
  %``Observation of electron-antineutrino disappearance at Daya Bay,''
  Phys.\ Rev.\ Lett.\  {\bf 108}, 171803 (2012)
  doi:10.1103/PhysRevLett.108.171803
  [arXiv:1203.1669 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.108.171803;%%
  %1491 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Abe:2011sj}
\bibitem{Abe:2011sj} 
  K.~Abe {\it et al.} [T2K Collaboration],
  %``Indication of Electron Neutrino Appearance from an Accelerator-produced Off-axis Muon Neutrino Beam,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 041801 (2011)
  doi:10.1103/PhysRevLett.107.041801
  [arXiv:1106.2822 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.107.041801;%%
  %1150 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Adamson:2011qu}
\bibitem{Adamson:2011qu} 
  P.~Adamson {\it et al.} [MINOS Collaboration],
  %``Improved search for muon-neutrino to electron-neutrino oscillations in MINOS,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 181802 (2011)
  doi:10.1103/PhysRevLett.107.181802
  [arXiv:1108.0015 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.107.181802;%%
  %640 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Abe:2011fz}
\bibitem{Abe:2011fz} 
  Y.~Abe {\it et al.} [Double Chooz Collaboration],
  %``Indication for the disappearance of reactor electron antineutrinos in the Double Chooz experiment,''
  Phys.\ Rev.\ Lett.\  {\bf 108}, 131801 (2012)
  doi:10.1103/PhysRevLett.108.131801
  [arXiv:1112.6353 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.108.131801;%%
  %842 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ahn:2012nd}
\bibitem{Ahn:2012nd} 
  J.~K.~Ahn {\it et al.} [RENO Collaboration],
  %``Observation of Reactor Electron Antineutrino Disappearance in the RENO Experiment,''
  Phys.\ Rev.\ Lett.\  {\bf 108}, 191802 (2012)
  doi:10.1103/PhysRevLett.108.191802
  [arXiv:1204.0626 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.108.191802;%%
  %1318 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Forero:2014bxa}
\bibitem{Forero:2014bxa} 
  D.~V.~Forero, M.~Tortola and J.~W.~F.~Valle,
  %``Neutrino oscillations refitted,''
  Phys.\ Rev.\ D {\bf 90}, no. 9, 093006 (2014)
  doi:10.1103/PhysRevD.90.093006
  [arXiv:1405.7540 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.093006;%%
  %281 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Fritzsch:1977za}
\bibitem{Fritzsch:1977za} 
  H.~Fritzsch,
  %``Calculating the Cabibbo Angle,''
  Phys.\ Lett.\ B {\bf 70}, 436 (1977).
  doi:10.1016/0370-2693(77)90408-7
  %%CITATION = doi:10.1016/0370-2693(77)90408-7;%%
  %540 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Fukuyama:1997ky}
\bibitem{Fukuyama:1997ky} 
  T.~Fukuyama and H.~Nishiura,
  %``Mass matrix of Majorana neutrinos,''
  hep-ph/9702253.
  %%CITATION = HEP-PH/9702253;%%
  %209 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Du:1992iy}
\bibitem{Du:1992iy} 
  D.~s.~Du and Z.~z.~Xing,
  %``A Modified Fritzsch ansatz with additional first order perturbation,''
  Phys.\ Rev.\ D {\bf 48}, 2349 (1993).
  doi:10.1103/PhysRevD.48.2349
  %%CITATION = doi:10.1103/PhysRevD.48.2349;%%
  %82 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Barbieri:1994kw}
\bibitem{Barbieri:1994kw} 
  R.~Barbieri, G.~R.~Dvali, A.~Strumia, Z.~Berezhiani and L.~J.~Hall,
  %``Flavor in supersymmetric grand unification: A Democratic approach,''
  Nucl.\ Phys.\ B {\bf 432}, 49 (1994)
  doi:10.1016/0550-3213(94)90593-2
  [hep-ph/9405428].
  %%CITATION = doi:10.1016/0550-3213(94)90593-2;%%
  %81 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Peccei:1995fg}
\bibitem{Peccei:1995fg} 
  R.~D.~Peccei and K.~Wang,
  %``Natural mass matrices,''
  Phys.\ Rev.\ D {\bf 53}, 2712 (1996)
  doi:10.1103/PhysRevD.53.2712
  [hep-ph/9509242].
  %%CITATION = doi:10.1103/PhysRevD.53.2712;%%
  %45 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Fritzsch:1999ee}
\bibitem{Fritzsch:1999ee} 
  H.~Fritzsch and Z.~z.~Xing,
  %``Mass and flavor mixing schemes of quarks and leptons,''
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 45}, 1 (2000)
  doi:10.1016/S0146-6410(00)00102-2
  [hep-ph/9912358].
  %%CITATION = doi:10.1016/S0146-6410(00)00102-2;%%
  %446 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Roberts:2001zy}
\bibitem{Roberts:2001zy} 
  R.~G.~Roberts, A.~Romanino, G.~G.~Ross and L.~Velasco-Sevilla,
  %``Precision test of a fermion mass texture,''
  Nucl.\ Phys.\ B {\bf 615}, 358 (2001)
  doi:10.1016/S0550-3213(01)00408-4
  [hep-ph/0104088].
  %%CITATION = doi:10.1016/S0550-3213(01)00408-4;%%
  %129 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Nishiura:2002ei}
\bibitem{Nishiura:2002ei} 
  H.~Nishiura, K.~Matsuda, T.~Kikuchi and T.~Fukuyama,
  %``Phenomenological analysis of lepton and quark mass matrices,''
  Phys.\ Rev.\ D {\bf 65}, 097301 (2002)
  doi:10.1103/PhysRevD.65.097301
  [hep-ph/0202189].
  %%CITATION = doi:10.1103/PhysRevD.65.097301;%%
  %25 citations counted in INSPIRE as of 28 Apr 2016



%\cite{deMedeirosVarzielas:2005ax}
\bibitem{deMedeirosVarzielas:2005ax} 
  I.~de Medeiros Varzielas and G.~G.~Ross,
  %``SU(3) family symmetry and neutrino bi-tri-maximal mixing,''
  Nucl.\ Phys.\ B {\bf 733}, 31 (2006)
  doi:10.1016/j.nuclphysb.2005.10.039
  [hep-ph/0507176].
  %%CITATION = doi:10.1016/j.nuclphysb.2005.10.039;%%
  %196 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Carcamo:2006dp}
\bibitem{Carcamo:2006dp} 
  A.~E.~Carcamo Hernandez, R.~Martinez and J.~A.~Rodriguez,
  %``Different kind of textures of Yukawa coupling matrices in the two Higgs doublet model type III,''
  Eur.\ Phys.\ J.\ C {\bf 50}, 935 (2007)
  doi:10.1140/epjc/s10052-007-0264-0
  [hep-ph/0606190].
  %%CITATION = doi:10.1140/epjc/s10052-007-0264-0;%%
  %36 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Kajiyama:2007gx}
\bibitem{Kajiyama:2007gx} 
  Y.~Kajiyama, M.~Raidal and A.~Strumia,
  %``The Golden ratio prediction for the solar neutrino mixing,''
  Phys.\ Rev.\ D {\bf 76}, 117301 (2007)
  doi:10.1103/PhysRevD.76.117301
  [arXiv:0705.4559 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.76.117301;%%
  %116 citations counted in INSPIRE as of 28 Apr 2016



%\cite{CarcamoHernandez:2010im}
\bibitem{CarcamoHernandez:2010im} 
  A.~E.~Carcamo Hernandez and R.~Rahman,
  %``A SUSY  GUT model with pseudo-Goldstone Higgs doublets,''
  Rev.\ Mex.\ Fis.\  {\bf 62}, no. 2, 100 (2016)
  [arXiv:1007.0447 [hep-ph]].
  %%CITATION = ARXIV:1007.0447;%%
  %15 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Branco:2010tx}
\bibitem{Branco:2010tx} 
  G.~C.~Branco, D.~Emmanuel-Costa and C.~Simoes,
  %``Nearest-Neighbour Interaction from an Abelian Symmetry and Deviations from Hermiticity,''
  Phys.\ Lett.\ B {\bf 690}, 62 (2010)
  doi:10.1016/j.physletb.2010.05.009
  [arXiv:1001.5065 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2010.05.009;%%
  %30 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Leser:2011fz}
\bibitem{Leser:2011fz} 
  P.~Leser and H.~Pas,
  %``Neutrino mass hierarchy and the origin of leptonic flavor mixing from the righthanded sector,''
  Phys.\ Rev.\ D {\bf 84}, 017303 (2011)
  doi:10.1103/PhysRevD.84.017303
  [arXiv:1104.2448 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.84.017303;%%
  %6 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Gupta:2012dma}
\bibitem{Gupta:2012dma} 
  M.~Gupta and G.~Ahuja,
  %``Flavor mixings and textures of the fermion mass matrices,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 27}, 1230033 (2012)
  doi:10.1142/S0217751X12300335
  [arXiv:1302.4823 [hep-ph]].
  %%CITATION = doi:10.1142/S0217751X12300335;%%
  %35 citations counted in INSPIRE as of 28 Apr 2016



%\cite{CarcamoHernandez:2012xy}
\bibitem{CarcamoHernandez:2012xy} 
  A.~E.~Carcamo Hernandez, C.~O.~Dib, N.~Neill H and A.~R.~Zerwekh,
  %``Quark masses and mixings in the RS1 model with a condensing 4th generation,''
  JHEP {\bf 1202}, 132 (2012)
  doi:10.1007/JHEP02(2012)132
  [arXiv:1201.0878 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP02(2012)132;%%
  %25 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2013mcf}
\bibitem{Hernandez:2013mcf} 
  A.~E.~Carcamo Hernandez, R.~Martinez and F.~Ochoa,
  %``Radiative seesaw-type mechanism of quark masses in $SU(3)_C \otimes SU(3)_L \otimes U(1)_X$,''
  Phys.\ Rev.\ D {\bf 87}, no. 7, 075009 (2013)
  doi:10.1103/PhysRevD.87.075009
  [arXiv:1302.1757 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.87.075009;%%
  %19 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Pas:2014bra}
\bibitem{Pas:2014bra} 
  H.~Päs and E.~Schumacher,
  %``Leptogenesis and $CP$ violation in $SU(5)$ models with lepton flavor mixing originating from the right-handed sector,''
  Phys.\ Rev.\ D {\bf 89}, no. 9, 096010 (2014)
  doi:10.1103/PhysRevD.89.096010
  [arXiv:1401.2328 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.096010;%%
  %6 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2014hka}
\bibitem{Hernandez:2014hka} 
  A.~E.~Carcamo Hernandez, S.~Kovalenko and I.~Schmidt,
  %``An SU(5) grand unified model with discrete flavour symmetries,''
  arXiv:1411.2913 [hep-ph].
  %%CITATION = ARXIV:1411.2913;%%
  %9 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2014zsa}
\bibitem{Hernandez:2014zsa} 
  A.~E.~C.~Hernández and I.~d.~M.~Varzielas,
  %``Viable textures for the fermion sector,''
  J.\ Phys.\ G {\bf 42}, no. 6, 065002 (2015)
  doi:10.1088/0954-3899/42/6/065002
  [arXiv:1410.2481 [hep-ph]].
  %%CITATION = doi:10.1088/0954-3899/42/6/065002;%%
  %13 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Nishiura:2014psa}
\bibitem{Nishiura:2014psa} 
  H.~Nishiura and T.~Fukuyama,
  %``Simple neutrino mass matrix with only two free parameters,''
  Mod.\ Phys.\ Lett.\ A {\bf 29}, 0147 (2014)
  doi:10.1142/S0217732314501478
  [arXiv:1405.2416 [hep-ph]].
  %%CITATION = doi:10.1142/S0217732314501478;%%
  %6 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Frank:2014aca}
\bibitem{Frank:2014aca} 
  M.~Frank, C.~Hamzaoui, N.~Pourtolami and M.~Toharia,
  %``Unified Flavor Symmetry from warped dimensions,''
  Phys.\ Lett.\ B {\bf 742}, 178 (2015)
  doi:10.1016/j.physletb.2015.01.025
  [arXiv:1406.2331 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2015.01.025;%%
  %8 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Sinha:2015ooa}
\bibitem{Sinha:2015ooa} 
  R.~Sinha, R.~Samanta and A.~Ghosal,
  %``Revisiting Allowed Two Zero Textures of Neutrino Mass Matrices through Linear and Inverse Seesaw,''
  arXiv:1508.05227 [hep-ph].
  %%CITATION = ARXIV:1508.05227;%%
  %6 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Nishiura:2015qia}
\bibitem{Nishiura:2015qia} 
  H.~Nishiura and T.~Fukuyama,
  %``Simple mass matrices of neutrinos and quarks consistent with observed mixings and masses,''
  Phys.\ Lett.\ B {\bf 753}, 57 (2016)
  doi:10.1016/j.physletb.2015.11.080
  [arXiv:1510.01035 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2015.11.080;%%
  %5 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Gautam:2015kya}
\bibitem{Gautam:2015kya} 
  R.~R.~Gautam, M.~Singh and M.~Gupta,
  %``Neutrino mass matrices with one texture zero and a vanishing neutrino mass,''
  Phys.\ Rev.\ D {\bf 92}, no. 1, 013006 (2015)
  doi:10.1103/PhysRevD.92.013006
  [arXiv:1506.04868 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.013006;%%
  %11 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Pas:2015hca}
\bibitem{Pas:2015hca} 
  H.~Päs and E.~Schumacher,
  %``Common origin of $R_K$ and neutrino masses,''
  Phys.\ Rev.\ D {\bf 92}, no. 11, 114025 (2015)
  doi:10.1103/PhysRevD.92.114025
  [arXiv:1510.08757 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.114025;%%
  %8 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2015hrt}
\bibitem{Hernandez:2015hrt} 
  A.~E.~C.~Hernández,
  %``The 750 GeV diphoton resonance can cause the SM fermion mass and mixing pattern,''
  arXiv:1512.09092 [hep-ph].
  %%CITATION = ARXIV:1512.09092;%%
  %60 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ishimori:2010au}
\bibitem{Ishimori:2010au} 
  H.~Ishimori, T.~Kobayashi, H.~Ohki, Y.~Shimizu, H.~Okada and M.~Tanimoto,
  %``Non-Abelian Discrete Symmetries in Particle Physics,''
  Prog.\ Theor.\ Phys.\ Suppl.\  {\bf 183}, 1 (2010)
  doi:10.1143/PTPS.183.1
  [arXiv:1003.3552 [hep-th]].
  %%CITATION = doi:10.1143/PTPS.183.1;%%
  %395 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Altarelli:2010gt}
\bibitem{Altarelli:2010gt} 
  G.~Altarelli and F.~Feruglio,
  %``Discrete Flavor Symmetries and Models of Neutrino Mixing,''
  Rev.\ Mod.\ Phys.\  {\bf 82}, 2701 (2010)
  doi:10.1103/RevModPhys.82.2701
  [arXiv:1002.0211 [hep-ph]].
  %%CITATION = doi:10.1103/RevModPhys.82.2701;%%
  %454 citations counted in INSPIRE as of 28 Apr 2016



%\cite{King:2013eh}
\bibitem{King:2013eh} 
  S.~F.~King and C.~Luhn,
  %``Neutrino Mass and Mixing with Discrete Symmetry,''
  Rept.\ Prog.\ Phys.\  {\bf 76}, 056201 (2013)
  doi:10.1088/0034-4885/76/5/056201
  [arXiv:1301.1340 [hep-ph]].
  %%CITATION = doi:10.1088/0034-4885/76/5/056201;%%
  %272 citations counted in INSPIRE as of 28 Apr 2016



%\cite{King:2014nza}
\bibitem{King:2014nza} 
  S.~F.~King, A.~Merle, S.~Morisi, Y.~Shimizu and M.~Tanimoto,
  %``Neutrino Mass and Mixing: from Theory to Experiment,''
  New J.\ Phys.\  {\bf 16}, 045018 (2014)
  doi:10.1088/1367-2630/16/4/045018
  [arXiv:1402.4271 [hep-ph]].
  %%CITATION = doi:10.1088/1367-2630/16/4/045018;%%
  %115 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ma:2001dn}
\bibitem{Ma:2001dn} 
  E.~Ma and G.~Rajasekaran,
  %``Softly broken A(4) symmetry for nearly degenerate neutrino masses,''
  Phys.\ Rev.\ D {\bf 64}, 113012 (2001)
  doi:10.1103/PhysRevD.64.113012
  [hep-ph/0106291].
  %%CITATION = doi:10.1103/PhysRevD.64.113012;%%
  %573 citations counted in INSPIRE as of 28 Apr 2016



%\cite{He:2006dk}
\bibitem{He:2006dk} 
  X.~G.~He, Y.~Y.~Keum and R.~R.~Volkas,
  %``A(4) flavor symmetry breaking scheme for understanding quark and neutrino mixing angles,''
  JHEP {\bf 0604}, 039 (2006)
  doi:10.1088/1126-6708/2006/04/039
  [hep-ph/0601001].
  %%CITATION = doi:10.1088/1126-6708/2006/04/039;%%
  %234 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Chen:2009um}
\bibitem{Chen:2009um} 
  M.~C.~Chen and S.~F.~King,
  %``A4 See-Saw Models and Form Dominance,''
  JHEP {\bf 0906}, 072 (2009)
  doi:10.1088/1126-6708/2009/06/072
  [arXiv:0903.0125 [hep-ph]].
  %%CITATION = doi:10.1088/1126-6708/2009/06/072;%%
  %111 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dong:2010gk}
\bibitem{Dong:2010gk} 
  P.~V.~Dong, L.~T.~Hue, H.~N.~Long and D.~V.~Soa,
  %``The 3-3-1 model with A_4 flavor symmetry,''
  Phys.\ Rev.\ D {\bf 81}, 053004 (2010)
  doi:10.1103/PhysRevD.81.053004
  [arXiv:1001.4625 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.81.053004;%%
  %37 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ahn:2012tv}
\bibitem{Ahn:2012tv} 
  Y.~H.~Ahn and S.~K.~Kang,
  %``Non-zero $\theta_{13}$ and CP violation in a model with $A_4$ flavor symmetry,''
  Phys.\ Rev.\ D {\bf 86}, 093003 (2012)
  doi:10.1103/PhysRevD.86.093003
  [arXiv:1203.4185 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.093003;%%
  %40 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Memenga:2013vc}
\bibitem{Memenga:2013vc} 
  N.~Memenga, W.~Rodejohann and H.~Zhang,
  %``$A_4$ flavor symmetry model for Dirac neutrinos and sizable $U_{e3}$,''
  Phys.\ Rev.\ D {\bf 87}, no. 5, 053021 (2013)
  doi:10.1103/PhysRevD.87.053021
  [arXiv:1301.2963 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.87.053021;%%
  %21 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Felipe:2013vwa}
\bibitem{Felipe:2013vwa} 
  R.~Gonzalez Felipe, H.~Serodio and J.~P.~Silva,
  %``Neutrino masses and mixing in A4 models with three Higgs doublets,''
  Phys.\ Rev.\ D {\bf 88}, no. 1, 015015 (2013)
  doi:10.1103/PhysRevD.88.015015
  [arXiv:1304.3468 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.015015;%%
  %17 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Varzielas:2012ai}
\bibitem{Varzielas:2012ai} 
  I.~de Medeiros Varzielas and D.~Pidt,
  %``UV completions of flavour models and large theta_{13},''
  JHEP {\bf 1303}, 065 (2013)
  doi:10.1007/JHEP03(2013)065
  [arXiv:1211.5370 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP03(2013)065;%%
  %21 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ishimori:2012fg}
\bibitem{Ishimori:2012fg} 
  H.~Ishimori and E.~Ma,
  %``New Simple $A_4$ Neutrino Model for Nonzero $\theta_{13}$ and Large $\delta_{CP}$,''
  Phys.\ Rev.\ D {\bf 86}, 045030 (2012)
  doi:10.1103/PhysRevD.86.045030
  [arXiv:1205.0075 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.045030;%%
  %46 citations counted in INSPIRE as of 28 Apr 2016



%\cite{King:2013hj}
\bibitem{King:2013hj} 
  S.~F.~King, S.~Morisi, E.~Peinado and J.~W.~F.~Valle,
  %``Quark-Lepton Mass Relation in a Realistic $A_4$ Extension of the Standard Model,''
  Phys.\ Lett.\ B {\bf 724}, 68 (2013)
  doi:10.1016/j.physletb.2013.05.067
  [arXiv:1301.7065 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2013.05.067;%%
  %25 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2013dta}
\bibitem{Hernandez:2013dta} 
  A.~E.~Carcamo Hernandez, I.~de Medeiros Varzielas, S.~G.~Kovalenko, H.~Päs and I.~Schmidt,
  %``Lepton masses and mixings in an $A_4$ multi-Higgs model with a radiative seesaw mechanism,''
  Phys.\ Rev.\ D {\bf 88}, no. 7, 076014 (2013)
  doi:10.1103/PhysRevD.88.076014
  [arXiv:1307.6499 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.076014;%%
  %40 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Babu:2002dz}
\bibitem{Babu:2002dz} 
  K.~S.~Babu, E.~Ma and J.~W.~F.~Valle,
  %``Underlying A(4) symmetry for the neutrino mass matrix and the quark mixing matrix,''
  Phys.\ Lett.\ B {\bf 552}, 207 (2003)
  doi:10.1016/S0370-2693(02)03153-2
  [hep-ph/0206292].
  %%CITATION = doi:10.1016/S0370-2693(02)03153-2;%%
  %563 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Altarelli:2005yx}
\bibitem{Altarelli:2005yx} 
  G.~Altarelli and F.~Feruglio,
  %``Tri-bimaximal neutrino mixing, A(4) and the modular symmetry,''
  Nucl.\ Phys.\ B {\bf 741}, 215 (2006)
  doi:10.1016/j.nuclphysb.2006.02.015
  [hep-ph/0512103].
  %%CITATION = doi:10.1016/j.nuclphysb.2006.02.015;%%
  %467 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Morisi:2013eca}
\bibitem{Morisi:2013eca} 
  S.~Morisi, M.~Nebot, K.~M.~Patel, E.~Peinado and J.~W.~F.~Valle,
  %``Quark-Lepton Mass Relation and CKM mixing in an A4 Extension of the Minimal Supersymmetric Standard Model,''
  Phys.\ Rev.\ D {\bf 88}, 036001 (2013)
  doi:10.1103/PhysRevD.88.036001
  [arXiv:1303.4394 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.036001;%%
  %17 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Altarelli:2005yp}
\bibitem{Altarelli:2005yp} 
  G.~Altarelli and F.~Feruglio,
  %``Tri-bimaximal neutrino mixing from discrete symmetry in extra dimensions,''
  Nucl.\ Phys.\ B {\bf 720}, 64 (2005)
  doi:10.1016/j.nuclphysb.2005.05.005
  [hep-ph/0504165].
  %%CITATION = doi:10.1016/j.nuclphysb.2005.05.005;%%
  %473 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Kadosh:2010rm}
\bibitem{Kadosh:2010rm} 
  A.~Kadosh and E.~Pallante,
  %``An A(4) flavor model for quarks and leptons in warped geometry,''
  JHEP {\bf 1008}, 115 (2010)
  doi:10.1007/JHEP08(2010)115
  [arXiv:1004.0321 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2010)115;%%
  %45 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Kadosh:2013nra}
\bibitem{Kadosh:2013nra} 
  A.~Kadosh,
  %``$\Theta_13$ and charged Lepton Flavor Violation in "warped" $A_4$ models,''
  JHEP {\bf 1306}, 114 (2013)
  doi:10.1007/JHEP06(2013)114
  [arXiv:1303.2645 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2013)114;%%
  %8 citations counted in INSPIRE as of 28 Apr 2016



%\cite{delAguila:2010vg}
\bibitem{delAguila:2010vg} 
  F.~del Aguila, A.~Carmona and J.~Santiago,
  %``Neutrino Masses from an A4 Symmetry in Holographic Composite Higgs Models,''
  JHEP {\bf 1008}, 127 (2010)
  doi:10.1007/JHEP08(2010)127
  [arXiv:1001.5151 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2010)127;%%
  %66 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Campos:2014lla}
\bibitem{Campos:2014lla} 
  M.~D.~Campos, A.~E.~Cárcamo Hernández, S.~Kovalenko, I.~Schmidt and E.~Schumacher,
  %``Fermion masses and mixings in an $SU(5)$ grand unified model with an extra flavor symmetry,''
  Phys.\ Rev.\ D {\bf 90}, no. 1, 016006 (2014)
  doi:10.1103/PhysRevD.90.016006
  [arXiv:1403.2525 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.016006;%%
  %19 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Vien:2014pta}
\bibitem{Vien:2014pta} 
  V.~V.~Vien and H.~N.~Long,
  %``Neutrino mixing with nonzero $\theta_{13}$ and CP violation in the 3-3-1 model based on $A_4$ flavor symmetry,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 30}, no. 21, 1550117 (2015)
  doi:10.1142/S0217751X15501171
  [arXiv:1405.4665 [hep-ph]].
  %%CITATION = doi:10.1142/S0217751X15501171;%%
  %8 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2015tna}
\bibitem{Hernandez:2015tna} 
  A.~E.~Cárcamo Hernández and R.~Martinez,
  %``A predictive 3-3-1 model with $A_4$ flavor symmetry,''
  Nucl.\ Phys.\ B {\bf 905}, 337 (2016)
  doi:10.1016/j.nuclphysb.2016.02.025
  [arXiv:1501.05937 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2016.02.025;%%
  %13 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Nishi:2016jqg}
\bibitem{Nishi:2016jqg} 
  C.~C.~Nishi,
  %``A New and Trivial CP Symmetry for Extended $A_4$ Flavor,''
  arXiv:1601.00977 [hep-ph].
  %%CITATION = ARXIV:1601.00977;%%
  %2 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Chen:2004rr}
\bibitem{Chen:2004rr} 
  S.~L.~Chen, M.~Frigerio and E.~Ma,
  %``Large neutrino mixing and normal mass hierarchy: A Discrete understanding,''
  Phys.\ Rev.\ D {\bf 70}, 073008 (2004)
  Erratum: [Phys.\ Rev.\ D {\bf 70}, 079905 (2004)]
  doi:10.1103/PhysRevD.70.079905, 10.1103/PhysRevD.70.073008
  [hep-ph/0404084].
  %%CITATION = doi:10.1103/PhysRevD.70.079905, 10.1103/PhysRevD.70.073008;%%
  %129 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dong:2011vb}
\bibitem{Dong:2011vb} 
  P.~V.~Dong, H.~N.~Long, C.~H.~Nam and V.~V.~Vien,
  %``The $S_3$ flavor symmetry in 3-3-1 models,''
  Phys.\ Rev.\ D {\bf 85}, 053001 (2012)
  doi:10.1103/PhysRevD.85.053001
  [arXiv:1111.6360 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.85.053001;%%
  %42 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Bhattacharyya:2010hp}
\bibitem{Bhattacharyya:2010hp} 
  G.~Bhattacharyya, P.~Leser and H.~Pas,
  %``Exotic Higgs boson decay modes as a harbinger of $S_3$ flavor symmetry,''
  Phys.\ Rev.\ D {\bf 83}, 011701 (2011)
  doi:10.1103/PhysRevD.83.011701
  [arXiv:1006.5597 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.83.011701;%%
  %48 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2012bh}
\bibitem{Dias:2012bh} 
  A.~G.~Dias, A.~C.~B.~Machado and C.~C.~Nishi,
  %``An $S_3$ Model for Lepton Mass Matrices with Nearly Minimal Texture,''
  Phys.\ Rev.\ D {\bf 86}, 093005 (2012)
  doi:10.1103/PhysRevD.86.093005
  [arXiv:1206.6362 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.093005;%%
  %13 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Meloni:2012ci}
\bibitem{Meloni:2012ci} 
  D.~Meloni,
  %``$S_3$ as a flavour symmetry for quarks and leptons after the Daya Bay result on $\theta_{13}$,''
  JHEP {\bf 1205}, 124 (2012)
  doi:10.1007/JHEP05(2012)124
  [arXiv:1203.3126 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP05(2012)124;%%
  %22 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Canales:2013cga}
\bibitem{Canales:2013cga} 
  F.~González Canales, A.~Mondragón, M.~Mondragón, U.~J.~Saldaña Salazar and L.~Velasco-Sevilla,
  %``Quark sector of S3 models: classification and comparison with experimental data,''
  Phys.\ Rev.\ D {\bf 88}, 096004 (2013)
  doi:10.1103/PhysRevD.88.096004
  [arXiv:1304.6644 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.096004;%%
  %31 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ma:2013zca}
\bibitem{Ma:2013zca} 
  E.~Ma and B.~Melic,
  %``Updated $S_{3}$ model of quarks,''
  Phys.\ Lett.\ B {\bf 725}, 402 (2013)
  doi:10.1016/j.physletb.2013.07.015
  [arXiv:1303.6928 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2013.07.015;%%
  %24 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Kajiyama:2013sza}
\bibitem{Kajiyama:2013sza} 
  Y.~Kajiyama, H.~Okada and K.~Yagyu,
  %``Electron/Muon Specific Two Higgs Doublet Model,''
  Nucl.\ Phys.\ B {\bf 887}, 358 (2014)
  doi:10.1016/j.nuclphysb.2014.08.009
  [arXiv:1309.6234 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2014.08.009;%%
  %32 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2013hea}
\bibitem{Hernandez:2013hea} 
  A.~E.~Cárcamo Hernández, R.~Martínez and F.~Ochoa,
  %``Fermion masses and mixings in the 3-3-1 model with right-handed neutrinos based on the $S_3$ flavor symmetry,''
  arXiv:1309.6567 [hep-ph].
  %%CITATION = ARXIV:1309.6567;%%
  %29 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ma:2014qra}
\bibitem{Ma:2014qra} 
  E.~Ma and R.~Srivastava,
  %``Dirac or inverse seesaw neutrino masses with $B-L$ gauge symmetry and $S_3$ flavor symmetry,''
  Phys.\ Lett.\ B {\bf 741}, 217 (2015)
  doi:10.1016/j.physletb.2014.12.049
  [arXiv:1411.5042 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2014.12.049;%%
  %17 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2014vta}
\bibitem{Hernandez:2014vta} 
  A.~E.~C.~Hernández, R.~Martinez and J.~Nisperuza,
  %``$S_3$ discrete group as a source of the quark mass and mixing pattern in $331$ models,''
  Eur.\ Phys.\ J.\ C {\bf 75}, no. 2, 72 (2015)
  doi:10.1140/epjc/s10052-015-3278-z
  [arXiv:1401.0937 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-015-3278-z;%%
  %25 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2014lpa}
\bibitem{Hernandez:2014lpa} 
  A.~E.~C.~Hernández, E.~C.~Mur and R.~Martinez,
  %``Lepton masses and mixing in $SU(3)_{C}\otimes SU(3)_{L}\otimes U(1)_{X}$ models with a $S_3$ flavor symmetry,''
  Phys.\ Rev.\ D {\bf 90}, no. 7, 073001 (2014)
  doi:10.1103/PhysRevD.90.073001
  [arXiv:1407.5217 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.073001;%%
  %16 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2015dga}
\bibitem{Hernandez:2015dga} 
  A.~E.~Cárcamo Hernández, I.~de Medeiros Varzielas and E.~Schumacher,
  %``Fermion and scalar phenomenology of a two-Higgs-doublet model with $S_3$,''
  Phys.\ Rev.\ D {\bf 93}, no. 1, 016003 (2016)
  doi:10.1103/PhysRevD.93.016003
  [arXiv:1509.02083 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.93.016003;%%
  %12 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2015zeh}
\bibitem{Hernandez:2015zeh} 
  A.~E.~C.~Hernández, I.~d.~M.~Varzielas and N.~A.~Neill,
  %``A Novel Randall-Sundrum Model with $S_{3}$ Flavor Symmetry,''
  arXiv:1511.07420 [hep-ph].
  %%CITATION = ARXIV:1511.07420;%%
  %7 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2016rbi}
\bibitem{Hernandez:2016rbi} 
  A.~E.~C.~Hernández, I.~d.~M.~Varzielas and E.~Schumacher,
  %``The $750\,\text{GeV}$ diphoton resonance in the light of a 2HDM with $S_3$ flavour symmetry,''
  arXiv:1601.00661 [hep-ph].
  %%CITATION = ARXIV:1601.00661;%%
  %43 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Mohapatra:2012tb}
\bibitem{Mohapatra:2012tb} 
  R.~N.~Mohapatra and C.~C.~Nishi,
  %``$S_4$ Flavored CP Symmetry for Neutrinos,''
  Phys.\ Rev.\ D {\bf 86}, 073007 (2012)
  doi:10.1103/PhysRevD.86.073007
  [arXiv:1208.2875 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.073007;%%
  %59 citations counted in INSPIRE as of 28 Apr 2016



%\cite{BhupalDev:2012nm}
\bibitem{BhupalDev:2012nm} 
  P.~S.~Bhupal Dev, B.~Dutta, R.~N.~Mohapatra and M.~Severson,
  %``$\theta_{13}$ and Proton Decay in a Minimal $SO(10) \times S_4$ model of Flavor,''
  Phys.\ Rev.\ D {\bf 86}, 035002 (2012)
  doi:10.1103/PhysRevD.86.035002
  [arXiv:1202.4012 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.035002;%%
  %45 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Varzielas:2012pa}
\bibitem{Varzielas:2012pa} 
  I.~de Medeiros Varzielas and L.~Lavoura,
  %``Flavour models for $TM_{1}$ lepton mixing,''
  J.\ Phys.\ G {\bf 40}, 085002 (2013)
  doi:10.1088/0954-3899/40/8/085002
  [arXiv:1212.3247 [hep-ph]].
  %%CITATION = doi:10.1088/0954-3899/40/8/085002;%%
  %29 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ding:2013hpa}
\bibitem{Ding:2013hpa} 
  G.~J.~Ding, S.~F.~King, C.~Luhn and A.~J.~Stuart,
  %``Spontaneous CP violation from vacuum alignment in $S_4$ models of leptons,''
  JHEP {\bf 1305}, 084 (2013)
  doi:10.1007/JHEP05(2013)084
  [arXiv:1303.6180 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP05(2013)084;%%
  %59 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ishimori:2010fs}
\bibitem{Ishimori:2010fs} 
  H.~Ishimori, Y.~Shimizu, M.~Tanimoto and A.~Watanabe,
  %``Neutrino masses and mixing from $S_{4}$ flavor twisting,''
  Phys.\ Rev.\ D {\bf 83}, 033004 (2011)
  doi:10.1103/PhysRevD.83.033004
  [arXiv:1010.3805 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.83.033004;%%
  %45 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ding:2013eca}
\bibitem{Ding:2013eca} 
  G.~J.~Ding and Y.~L.~Zhou,
  %``Dirac Neutrinos with $S_4$ Flavor Symmetry in Warped Extra Dimensions,''
  Nucl.\ Phys.\ B {\bf 876}, 418 (2013)
  doi:10.1016/j.nuclphysb.2013.08.011
  [arXiv:1304.2645 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2013.08.011;%%
  %17 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hagedorn:2011un}
\bibitem{Hagedorn:2011un} 
  C.~Hagedorn and M.~Serone,
  %``Leptons in Holographic Composite Higgs Models with Non-Abelian Discrete Symmetries,''
  JHEP {\bf 1110}, 083 (2011)
  doi:10.1007/JHEP10(2011)083
  [arXiv:1106.4021 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2011)083;%%
  %20 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Campos:2014zaa}
\bibitem{Campos:2014zaa} 
  M.~D.~Campos, A.~E.~C.~Hernández, H.~Päs and E.~Schumacher,
  %``Higgs $\rightarrow$ $\mu\tau$ as an indication for $S_4$ flavor symmetry,''
  Phys.\ Rev.\ D {\bf 91}, no. 11, 116011 (2015)
  doi:10.1103/PhysRevD.91.116011
  [arXiv:1408.1652 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.91.116011;%%
  %45 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dong:2010zu}
\bibitem{Dong:2010zu} 
  P.~V.~Dong, H.~N.~Long, D.~V.~Soa and V.~V.~Vien,
  %``The 3-3-1 model with $S_4$ flavor symmetry,''
  Eur.\ Phys.\ J.\ C {\bf 71}, 1544 (2011)
  doi:10.1140/epjc/s10052-011-1544-2
  [arXiv:1009.2328 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-011-1544-2;%%
  %42 citations counted in INSPIRE as of 28 Apr 2016



%\cite{VanVien:2015xha}
\bibitem{VanVien:2015xha} 
  V.~V.~Vien, H.~N.~Long and D.~P.~Khoi,
  %``Neutrino Mixing with Non-Zero $\theta_{13}$ and CP Violation in the 3-3-1 Model Based on $S_4$ Flavor Symmetry,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 30}, no. 17, 1550102 (2015)
  doi:10.1142/S0217751X1550102X
  [arXiv:1506.06063 [hep-ph]].
  %%CITATION = doi:10.1142/S0217751X1550102X;%%
  %4 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Frampton:1994rk}
\bibitem{Frampton:1994rk} 
  P.~H.~Frampton and T.~W.~Kephart,
  %``Simple nonAbelian finite flavor groups and fermion masses,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 10}, 4689 (1995)
  doi:10.1142/S0217751X95002187
  [hep-ph/9409330].
  %%CITATION = doi:10.1142/S0217751X95002187;%%
  %147 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Grimus:2003kq}
\bibitem{Grimus:2003kq} 
  W.~Grimus and L.~Lavoura,
  %``A Discrete symmetry group for maximal atmospheric neutrino mixing,''
  Phys.\ Lett.\ B {\bf 572}, 189 (2003)
  doi:10.1016/j.physletb.2003.08.032
  [hep-ph/0305046].
  %%CITATION = doi:10.1016/j.physletb.2003.08.032;%%
  %240 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Grimus:2004rj}
\bibitem{Grimus:2004rj} 
  W.~Grimus, A.~S.~Joshipura, S.~Kaneko, L.~Lavoura and M.~Tanimoto,
  %``Lepton mixing angle $\theta_{13} = 0$ with a horizontal symmetry $D_4$,''
  JHEP {\bf 0407}, 078 (2004)
  doi:10.1088/1126-6708/2004/07/078
  [hep-ph/0407112].
  %%CITATION = doi:10.1088/1126-6708/2004/07/078;%%
  %115 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Frigerio:2004jg}
\bibitem{Frigerio:2004jg} 
  M.~Frigerio, S.~Kaneko, E.~Ma and M.~Tanimoto,
  %``Quaternion family symmetry of quarks and leptons,''
  Phys.\ Rev.\ D {\bf 71}, 011901 (2005)
  doi:10.1103/PhysRevD.71.011901
  [hep-ph/0409187].
  %%CITATION = doi:10.1103/PhysRevD.71.011901;%%
  %80 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Babu:2004tn}
\bibitem{Babu:2004tn} 
  K.~S.~Babu and J.~Kubo,
  %``Dihedral families of quarks, leptons and Higgses,''
  Phys.\ Rev.\ D {\bf 71}, 056006 (2005)
  doi:10.1103/PhysRevD.71.056006
  [hep-ph/0411226].
  %%CITATION = doi:10.1103/PhysRevD.71.056006;%%
  %120 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Adulpravitchai:2008yp}
\bibitem{Adulpravitchai:2008yp} 
  A.~Adulpravitchai, A.~Blum and C.~Hagedorn,
  %``A Supersymmetric D4 Model for mu-tau Symmetry,''
  JHEP {\bf 0903}, 046 (2009)
  doi:10.1088/1126-6708/2009/03/046
  [arXiv:0812.3799 [hep-ph]].
  %%CITATION = doi:10.1088/1126-6708/2009/03/046;%%
  %44 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ishimori:2008gp}
\bibitem{Ishimori:2008gp} 
  H.~Ishimori, T.~Kobayashi, H.~Ohki, Y.~Omura, R.~Takahashi and M.~Tanimoto,
  %``D(4) Flavor Symmetry for Neutrino Masses and Mixing,''
  Phys.\ Lett.\ B {\bf 662}, 178 (2008)
  doi:10.1016/j.physletb.2008.03.007
  [arXiv:0802.2310 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2008.03.007;%%
  %42 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hagedorn:2010mq}
\bibitem{Hagedorn:2010mq} 
  C.~Hagedorn and R.~Ziegler,
  %``$\mu-\tau$ Symmetry and Charged Lepton Mass Hierarchy in a Supersymmetric $D_4$ Model,''
  Phys.\ Rev.\ D {\bf 82}, 053011 (2010)
  doi:10.1103/PhysRevD.82.053011
  [arXiv:1007.1888 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.82.053011;%%
  %12 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Meloni:2011cc}
\bibitem{Meloni:2011cc} 
  D.~Meloni, S.~Morisi and E.~Peinado,
  %``Stability of dark matter from the D4xZ2 flavor group,''
  Phys.\ Lett.\ B {\bf 703}, 281 (2011)
  doi:10.1016/j.physletb.2011.07.084
  [arXiv:1104.0178 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2011.07.084;%%
  %23 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Vien:2013zra}
\bibitem{Vien:2013zra} 
  V.~V.~Vien and H.~N.~Long,
  %``The $D_4$ flavor symmery in 3-3-1 model with neutral leptons,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 28}, 1350159 (2013)
  doi:10.1142/S0217751X13501595
  [arXiv:1312.5034 [hep-ph]].
  %%CITATION = doi:10.1142/S0217751X13501595;%%
  %18 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Luhn:2007sy}
\bibitem{Luhn:2007sy} 
  C.~Luhn, S.~Nasri and P.~Ramond,
  %``Tri-bimaximal neutrino mixing and the family symmetry semidirect product of Z(7) and Z(3),''
  Phys.\ Lett.\ B {\bf 652}, 27 (2007)
  doi:10.1016/j.physletb.2007.06.059
  [arXiv:0706.2341 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2007.06.059;%%
  %143 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hagedorn:2008bc}
\bibitem{Hagedorn:2008bc} 
  C.~Hagedorn, M.~A.~Schmidt and A.~Y.~Smirnov,
  %``Lepton Mixing and Cancellation of the Dirac Mass Hierarchy in SO(10) GUTs with Flavor Symmetries T(7) and Sigma(81),''
  Phys.\ Rev.\ D {\bf 79}, 036002 (2009)
  doi:10.1103/PhysRevD.79.036002
  [arXiv:0811.2955 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.79.036002;%%
  %62 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Cao:2010mp}
\bibitem{Cao:2010mp} 
  Q.~H.~Cao, S.~Khalil, E.~Ma and H.~Okada,
  %``Observable $T_7$ Lepton Flavor Symmetry at the Large Hadron Collider,''
  Phys.\ Rev.\ Lett.\  {\bf 106}, 131801 (2011)
  doi:10.1103/PhysRevLett.106.131801
  [arXiv:1009.5415 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.106.131801;%%
  %32 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Luhn:2012bc}
\bibitem{Luhn:2012bc} 
  C.~Luhn, K.~M.~Parattu and A.~Wingerter,
  %``A Minimal Model of Neutrino Flavor,''
  JHEP {\bf 1212}, 096 (2012)
  doi:10.1007/JHEP12(2012)096
  [arXiv:1210.1197 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP12(2012)096;%%
  %23 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Kajiyama:2013lja}
\bibitem{Kajiyama:2013lja} 
  Y.~Kajiyama, H.~Okada and K.~Yagyu,
  %``$T_7$ Flavor Model in Three Loop Seesaw and Higgs Phenomenology,''
  JHEP {\bf 1310}, 196 (2013)
  doi:10.1007/JHEP10(2013)196
  [arXiv:1307.0480 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2013)196;%%
  %39 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Bonilla:2014xla}
\bibitem{Bonilla:2014xla} 
  C.~Bonilla, S.~Morisi, E.~Peinado and J.~W.~F.~Valle,
  %``Relating quarks and leptons with the $T_7$ flavour group,''
  Phys.\ Lett.\ B {\bf 742}, 99 (2015)
  doi:10.1016/j.physletb.2015.01.017
  [arXiv:1411.4883 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2015.01.017;%%
  %14 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Vien:2014gza}
\bibitem{Vien:2014gza} 
  V.~V.~Vien and H.~N.~Long,
  %``The $T_7$ flavor symmetry in 3-3-1 model with neutral leptons,''
  JHEP {\bf 1404}, 133 (2014)
  doi:10.1007/JHEP04(2014)133
  [arXiv:1402.1256 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP04(2014)133;%%
  %20 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Vien:2015koa}
\bibitem{Vien:2015koa} 
  V.~V.~Vien,
  %``$T_7$ flavor symmetry scheme for understanding neutrino mass and mixing in 3-3-1 model with neutral leptons,''
  Mod.\ Phys.\ Lett.\ A {\bf 29}, 28 (2014)
  doi:10.1142/S0217732314501399
  [arXiv:1508.02585 [hep-ph]].
  %%CITATION = doi:10.1142/S0217732314501399;%%
  %3 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2015cra}
\bibitem{Hernandez:2015cra} 
  A.~E.~C.~Hernández and R.~Martinez,
  %``Fermion mass and mixing pattern in a minimal T7 flavor 331 model,''
  J.\ Phys.\ G {\bf 43}, no. 4, 045003 (2016)
  doi:10.1088/0954-3899/43/4/045003
  [arXiv:1501.07261 [hep-ph]].
  %%CITATION = doi:10.1088/0954-3899/43/4/045003;%%
  %17 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Arbelaez:2015toa}
\bibitem{Arbelaez:2015toa} 
  C.~Arbeláez, A.~E.~Cárcamo Hernández, S.~Kovalenko and I.~Schmidt,
  %``Adjoint $SU(5)$ GUT model with $T_{7}$ flavor symmetry,''
  Phys.\ Rev.\ D {\bf 92}, no. 11, 115015 (2015)
  doi:10.1103/PhysRevD.92.115015
  [arXiv:1507.03852 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.115015;%%
  %8 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ding:2011qt}
\bibitem{Ding:2011qt} 
  G.~J.~Ding,
  %``Tri-Bimaximal Neutrino Mixing and the $T_{13}$ Flavor Symmetry,''
  Nucl.\ Phys.\ B {\bf 853}, 635 (2011)
  doi:10.1016/j.nuclphysb.2011.08.012
  [arXiv:1105.5879 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2011.08.012;%%
  %11 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hartmann:2011dn}
\bibitem{Hartmann:2011dn} 
  C.~Hartmann,
  %``The Frobenius group T13 and the canonical see-saw mechanism applied to neutrino mixing,''
  Phys.\ Rev.\ D {\bf 85}, 013012 (2012)
  doi:10.1103/PhysRevD.85.013012
  [arXiv:1109.5143 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.85.013012;%%
  %5 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hartmann:2011pq}
\bibitem{Hartmann:2011pq} 
  C.~Hartmann and A.~Zee,
  %``Neutrino Mixing and the Frobenius Group T13,''
  Nucl.\ Phys.\ B {\bf 853}, 105 (2011)
  doi:10.1016/j.nuclphysb.2011.07.023
  [arXiv:1106.0333 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2011.07.023;%%
  %9 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Kajiyama:2010sb}
\bibitem{Kajiyama:2010sb} 
  Y.~Kajiyama and H.~Okada,
  %``T(13) Flavor Symmetry and Decaying Dark Matter,''
  Nucl.\ Phys.\ B {\bf 848}, 303 (2011)
  doi:10.1016/j.nuclphysb.2011.02.020
  [arXiv:1011.5753 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2011.02.020;%%
  %32 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Aranda:2000tm}
\bibitem{Aranda:2000tm} 
  A.~Aranda, C.~D.~Carone and R.~F.~Lebed,
  %``Maximal neutrino mixing from a minimal flavor symmetry,''
  Phys.\ Rev.\ D {\bf 62}, 016009 (2000)
  doi:10.1103/PhysRevD.62.016009
  [hep-ph/0002044].
  %%CITATION = doi:10.1103/PhysRevD.62.016009;%%
  %110 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Aranda:2007dp}
\bibitem{Aranda:2007dp} 
  A.~Aranda,
  %``Neutrino mixing from the double tetrahedral group T-prime,''
  Phys.\ Rev.\ D {\bf 76}, 111301 (2007)
  doi:10.1103/PhysRevD.76.111301
  [arXiv:0707.3661 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.76.111301;%%
  %70 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Chen:2007afa}
\bibitem{Chen:2007afa} 
  M.~C.~Chen and K.~T.~Mahanthappa,
  %``CKM and Tri-bimaximal MNS Matrices in a $SU(5) \times ^{(d)}T$ Model,''
  Phys.\ Lett.\ B {\bf 652}, 34 (2007)
  doi:10.1016/j.physletb.2007.06.064
  [arXiv:0705.0714 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2007.06.064;%%
  %202 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Frampton:2008bz}
\bibitem{Frampton:2008bz} 
  P.~H.~Frampton, T.~W.~Kephart and S.~Matsuzaki,
  %``Simplified Renormalizable T-prime Model for Tribimaximal Mixing and Cabibbo Angle,''
  Phys.\ Rev.\ D {\bf 78}, 073004 (2008)
  doi:10.1103/PhysRevD.78.073004
  [arXiv:0807.4713 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.78.073004;%%
  %54 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Eby:2011ph}
\bibitem{Eby:2011ph} 
  D.~A.~Eby, P.~H.~Frampton, X.~G.~He and T.~W.~Kephart,
  %``Quartification with T' Flavor,''
  Phys.\ Rev.\ D {\bf 84}, 037302 (2011)
  doi:10.1103/PhysRevD.84.037302
  [arXiv:1103.5737 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.84.037302;%%
  %10 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Frampton:2013lva}
\bibitem{Frampton:2013lva} 
  P.~H.~Frampton, C.~M.~Ho and T.~W.~Kephart,
  %``Heterotic discrete flavor model,''
  Phys.\ Rev.\ D {\bf 89}, no. 2, 027701 (2014)
  doi:10.1103/PhysRevD.89.027701
  [arXiv:1305.4402 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.027701;%%
  %8 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ma:2007wu}
\bibitem{Ma:2007wu} 
  E.~Ma,
  %``Near tribimaximal neutrino mixing with Delta(27) symmetry,''
  Phys.\ Lett.\ B {\bf 660}, 505 (2008)
  doi:10.1016/j.physletb.2007.12.060
  [arXiv:0709.0507 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2007.12.060;%%
  %93 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Varzielas:2012nn}
\bibitem{Varzielas:2012nn} 
  I.~de Medeiros Varzielas, D.~Emmanuel-Costa and P.~Leser,
  %``Geometrical CP Violation from Non-Renormalisable Scalar Potentials,''
  Phys.\ Lett.\ B {\bf 716}, 193 (2012)
  doi:10.1016/j.physletb.2012.08.008
  [arXiv:1204.3633 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2012.08.008;%%
  %43 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Bhattacharyya:2012pi}
\bibitem{Bhattacharyya:2012pi} 
  G.~Bhattacharyya, I.~de Medeiros Varzielas and P.~Leser,
  %``A common origin of fermion mixing and geometrical CP violation, and its test through Higgs physics at the LHC,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 241603 (2012)
  doi:10.1103/PhysRevLett.109.241603
  [arXiv:1210.0545 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.109.241603;%%
  %56 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ma:2013xqa}
\bibitem{Ma:2013xqa} 
  E.~Ma,
  %``Neutrino Mixing and Geometric CP Violation with Delta(27) Symmetry,''
  Phys.\ Lett.\ B {\bf 723}, 161 (2013)
  doi:10.1016/j.physletb.2013.05.011
  [arXiv:1304.1603 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2013.05.011;%%
  %20 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Nishi:2013jqa}
\bibitem{Nishi:2013jqa} 
  C.~C.~Nishi,
  %``Generalized $CP$ symmetries in $\Delta(27)$ flavor models,''
  Phys.\ Rev.\ D {\bf 88}, no. 3, 033010 (2013)
  doi:10.1103/PhysRevD.88.033010
  [arXiv:1306.0877 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.033010;%%
  %30 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Varzielas:2013sla}
\bibitem{Varzielas:2013sla} 
  I.~de Medeiros Varzielas and D.~Pidt,
  %``Towards realistic models of quark masses with geometrical CP violation,''
  J.\ Phys.\ G {\bf 41}, 025004 (2014)
  doi:10.1088/0954-3899/41/2/025004
  [arXiv:1307.0711 [hep-ph]].
  %%CITATION = doi:10.1088/0954-3899/41/2/025004;%%
  %27 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Aranda:2013gga}
\bibitem{Aranda:2013gga} 
  A.~Aranda, C.~Bonilla, S.~Morisi, E.~Peinado and J.~W.~F.~Valle,
  %``Dirac neutrinos from flavor symmetry,''
  Phys.\ Rev.\ D {\bf 89}, no. 3, 033001 (2014)
  doi:10.1103/PhysRevD.89.033001
  [arXiv:1307.3553 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.033001;%%
  %15 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ma:2014eka}
\bibitem{Ma:2014eka} 
  E.~Ma and A.~Natale,
  %``Scotogenic $Z_2$ or $U(1)_D$ Model of Neutrino Mass with $\Delta(27)$ Symmetry,''
  Phys.\ Lett.\ B {\bf 734}, 403 (2014)
  doi:10.1016/j.physletb.2014.05.070
  [arXiv:1403.6772 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2014.05.070;%%
  %18 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Abbas:2014ewa}
\bibitem{Abbas:2014ewa} 
  M.~Abbas and S.~Khalil,
  %``Fermion masses and mixing in $\Delta(27)$ flavour model,''
  Phys.\ Rev.\ D {\bf 91}, no. 5, 053003 (2015)
  doi:10.1103/PhysRevD.91.053003
  [arXiv:1406.6716 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.91.053003;%%
  %6 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Abbas:2015zna}
\bibitem{Abbas:2015zna} 
  M.~Abbas, S.~Khalil, A.~Rashed and A.~Sil,
  %``Neutrino masses and deviation from tribimaximal mixing in Δ(27) model with inverse seesaw mechanism,''
  Phys.\ Rev.\ D {\bf 93}, no. 1, 013018 (2016)
  doi:10.1103/PhysRevD.93.013018
  [arXiv:1508.03727 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.93.013018;%%
  %4 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Varzielas:2015aua}
\bibitem{Varzielas:2015aua} 
  I.~de Medeiros Varzielas,
  %``$\Delta(27)$ family symmetry and neutrino mixing,''
  JHEP {\bf 1508}, 157 (2015)
  doi:10.1007/JHEP08(2015)157
  [arXiv:1507.00338 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2015)157;%%
  %7 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Bjorkeroth:2015uou}
\bibitem{Bjorkeroth:2015uou} 
  F.~Björkeroth, F.~J.~de Anda, I.~d.~M.~Varzielas and S.~F.~King,
  %``Towards a complete $\Delta(27) \times SO(10)$ SUSY GUT,''
  arXiv:1512.00850 [hep-ph].
  %%CITATION = ARXIV:1512.00850;%%
  %4 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Chen:2015jta}
\bibitem{Chen:2015jta} 
  P.~Chen, G.~J.~Ding, A.~D.~Rojas, C.~A.~Vaquera-Araujo and J.~W.~F.~Valle,
  %``Warped flavor symmetry predictions for neutrino physics,''
  JHEP {\bf 1601}, 007 (2016)
  doi:10.1007/JHEP01(2016)007
  [arXiv:1509.06683 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2016)007;%%
  %7 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Vien:2016tmh}
\bibitem{Vien:2016tmh} 
  V.~V.~Vien, A.~E.~C.~Hernández and H.~N.~Long,
  %``The $\Delta(27)$ flavor 3-3-1 model with neutral leptons,''
  arXiv:1601.03300 [hep-ph].
  %%CITATION = ARXIV:1601.03300;%%
  %5 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Georgi:1978bv}
\bibitem{Georgi:1978bv} 
  H.~Georgi and A.~Pais,
  %``Generalization of Gim: Horizontal and Vertical Flavor Mixing,''
  Phys.\ Rev.\ D {\bf 19}, 2746 (1979).
  doi:10.1103/PhysRevD.19.2746
  %%CITATION = doi:10.1103/PhysRevD.19.2746;%%
  %58 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Valle:1983dk}
\bibitem{Valle:1983dk} 
  J.~W.~F.~Valle and M.~Singer,
  %``Lepton Number Violation With Quasi Dirac Neutrinos,''
  Phys.\ Rev.\ D {\bf 28}, 540 (1983).
  doi:10.1103/PhysRevD.28.540
  %%CITATION = doi:10.1103/PhysRevD.28.540;%%
  %116 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Pisano:1991ee}
\bibitem{Pisano:1991ee} 
  F.~Pisano and V.~Pleitez,
  %``An SU(3) x U(1) model for electroweak interactions,''
  Phys.\ Rev.\ D {\bf 46}, 410 (1992)
  doi:10.1103/PhysRevD.46.410
  [hep-ph/9206242].
  %%CITATION = doi:10.1103/PhysRevD.46.410;%%
  %538 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Montero:1992jk}
\bibitem{Montero:1992jk} 
  J.~C.~Montero, F.~Pisano and V.~Pleitez,
  %``Neutral currents and GIM mechanism in SU(3)-L x U(1)-N models for electroweak interactions,''
  Phys.\ Rev.\ D {\bf 47}, 2918 (1993)
  doi:10.1103/PhysRevD.47.2918
  [hep-ph/9212271].
  %%CITATION = doi:10.1103/PhysRevD.47.2918;%%
  %209 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Foot:1992rh}
\bibitem{Foot:1992rh} 
  R.~Foot, O.~F.~Hernandez, F.~Pisano and V.~Pleitez,
  %``Lepton masses in an SU(3)-L x U(1)-N gauge model,''
  Phys.\ Rev.\ D {\bf 47}, 4158 (1993)
  doi:10.1103/PhysRevD.47.4158
  [hep-ph/9207264].
  %%CITATION = doi:10.1103/PhysRevD.47.4158;%%
  %272 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Frampton:1992wt}
\bibitem{Frampton:1992wt} 
  P.~H.~Frampton,
  %``Chiral dilepton model and the flavor question,''
  Phys.\ Rev.\ Lett.\  {\bf 69}, 2889 (1992).
  doi:10.1103/PhysRevLett.69.2889
  %%CITATION = doi:10.1103/PhysRevLett.69.2889;%%
  %545 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ng:1992st}
\bibitem{Ng:1992st} 
  D.~Ng,
  %``The Electroweak theory of SU(3) x U(1),''
  Phys.\ Rev.\ D {\bf 49}, 4805 (1994)
  doi:10.1103/PhysRevD.49.4805
  [hep-ph/9212284].
  %%CITATION = doi:10.1103/PhysRevD.49.4805;%%
  %159 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Duong:1993zn}
\bibitem{Duong:1993zn} 
  T.~V.~Duong and E.~Ma,
  %``Supersymmetric SU(3) x U(1) gauge models: Higgs structure at the electroweak energy scale,''
  Phys.\ Lett.\ B {\bf 316}, 307 (1993)
  doi:10.1016/0370-2693(93)90329-G
  [hep-ph/9306264].
  %%CITATION = doi:10.1016/0370-2693(93)90329-G;%%
  %68 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hoang:1996gi}
\bibitem{Hoang:1996gi} 
  H.~N.~Long,
  %``SU(3)-L x U(1)-N model for right-handed neutrino neutral currents,''
  Phys.\ Rev.\ D {\bf 54}, 4691 (1996)
  doi:10.1103/PhysRevD.54.4691
  [hep-ph/9607439].
  %%CITATION = doi:10.1103/PhysRevD.54.4691;%%
  %166 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hoang:1995vq}
\bibitem{Hoang:1995vq} 
  H.~N.~Long,
  %``The 331 model with right handed neutrinos,''
  Phys.\ Rev.\ D {\bf 53}, 437 (1996)
  doi:10.1103/PhysRevD.53.437
  [hep-ph/9504274].
  %%CITATION = doi:10.1103/PhysRevD.53.437;%%
  %180 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Foot:1994ym}
\bibitem{Foot:1994ym} 
  R.~Foot, H.~N.~Long and T.~A.~Tran,
  %``SU(3)-L x U(1)-N and SU(4)-L x U(1)-N gauge models with right-handed neutrinos,''
  Phys.\ Rev.\ D {\bf 50}, 34 (1994)
  doi:10.1103/PhysRevD.50.R34
  [hep-ph/9402243].
  %%CITATION = doi:10.1103/PhysRevD.50.R34;%%
  %246 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Diaz:2003dk}
\bibitem{Diaz:2003dk} 
  R.~A.~Diaz, R.~Martinez and F.~Ochoa,
  %``The Scalar sector of the SU(3)(c) x SU(3)(L) x U(1)(X) model,''
  Phys.\ Rev.\ D {\bf 69}, 095009 (2004)
  doi:10.1103/PhysRevD.69.095009
  [hep-ph/0309280].
  %%CITATION = doi:10.1103/PhysRevD.69.095009;%%
  %70 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Diaz:2004fs}
\bibitem{Diaz:2004fs} 
  R.~A.~Diaz, R.~Martinez and F.~Ochoa,
  %``SU(3)(c) x SU(3)(L) x U(1)(X) models for beta arbitrary and families with mirror fermions,''
  Phys.\ Rev.\ D {\bf 72}, 035018 (2005)
  doi:10.1103/PhysRevD.72.035018
  [hep-ph/0411263].
  %%CITATION = doi:10.1103/PhysRevD.72.035018;%%
  %67 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2004dc}
\bibitem{Dias:2004dc} 
  A.~G.~Dias, R.~Martinez and V.~Pleitez,
  %``Concerning the Landau pole in 3-3-1 models,''
  Eur.\ Phys.\ J.\ C {\bf 39}, 101 (2005)
  doi:10.1140/epjc/s2004-02083-0
  [hep-ph/0407141].
  %%CITATION = doi:10.1140/epjc/s2004-02083-0;%%
  %69 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2005yh}
\bibitem{Dias:2005yh} 
  A.~G.~Dias, C.~A.~de S.Pires and P.~S.~Rodrigues da Silva,
  %``Naturally light right-handed neutrinos in a 3-3-1 model,''
  Phys.\ Lett.\ B {\bf 628}, 85 (2005)
  doi:10.1016/j.physletb.2005.09.028
  [hep-ph/0508186].
  %%CITATION = doi:10.1016/j.physletb.2005.09.028;%%
  %57 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2005jm}
\bibitem{Dias:2005jm} 
  A.~G.~Dias, A.~Doff, C.~A.~de S.Pires and P.~S.~Rodrigues da Silva,
  %``Neutrino decay and neutrinoless double beta decay in a 3-3-1 model,''
  Phys.\ Rev.\ D {\bf 72}, 035006 (2005)
  doi:10.1103/PhysRevD.72.035006
  [hep-ph/0503014].
  %%CITATION = doi:10.1103/PhysRevD.72.035006;%%
  %26 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ochoa:2005ch}
\bibitem{Ochoa:2005ch} 
  F.~Ochoa and R.~Martinez,
  %``Family dependence in SU(3)(c) x SU(3)(L) x U(1)(X) models,''
  Phys.\ Rev.\ D {\bf 72}, 035010 (2005)
  doi:10.1103/PhysRevD.72.035010
  [hep-ph/0505027].
  %%CITATION = doi:10.1103/PhysRevD.72.035010;%%
  %33 citations counted in INSPIRE as of 28 Apr 2016



%\cite{CarcamoHernandez:2005ka}
\bibitem{CarcamoHernandez:2005ka} 
  A.~E.~Carcamo Hernandez, R.~Martinez and F.~Ochoa,
  %``Z and Z' decays with and without FCNC in 331 models,''
  Phys.\ Rev.\ D {\bf 73}, 035007 (2006)
  doi:10.1103/PhysRevD.73.035007
  [hep-ph/0510421].
  %%CITATION = doi:10.1103/PhysRevD.73.035007;%%
  %60 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2010vt}
\bibitem{Dias:2010vt} 
  A.~G.~Dias, C.~A.~de S.Pires and P.~S.~Rodrigues da Silva,
  %``The Left-Right SU(3)(L)xSU(3)(R)xU(1)(X) Model with Light, keV and Heavy Neutrinos,''
  Phys.\ Rev.\ D {\bf 82}, 035013 (2010)
  doi:10.1103/PhysRevD.82.035013
  [arXiv:1003.3260 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.82.035013;%%
  %12 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2012xp}
\bibitem{Dias:2012xp} 
  A.~G.~Dias, C.~A.~de S.Pires, P.~S.~Rodrigues da Silva and A.~Sampieri,
  %``A Simple Realization of the Inverse Seesaw Mechanism,''
  Phys.\ Rev.\ D {\bf 86}, 035007 (2012)
  doi:10.1103/PhysRevD.86.035007
  [arXiv:1206.2590].
  %%CITATION = doi:10.1103/PhysRevD.86.035007;%%
  %20 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Alvarado:2012xi}
\bibitem{Alvarado:2012xi} 
  C.~Alvarado, R.~Martinez and F.~Ochoa,
  %``Quark mass hierarchy in 3-3-1 models,''
  Phys.\ Rev.\ D {\bf 86}, 025027 (2012)
  doi:10.1103/PhysRevD.86.025027
  [arXiv:1207.0014 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.025027;%%
  %15 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Catano:2012kw}
\bibitem{Catano:2012kw} 
  M.~E.~Catano, R.~Martinez and F.~Ochoa,
  %``Neutrino masses in a 331 model with right-handed neutrinos without doubly charged Higgs bosons via inverse and double seesaw mechanisms,''
  Phys.\ Rev.\ D {\bf 86}, 073015 (2012)
  doi:10.1103/PhysRevD.86.073015
  [arXiv:1206.1966 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.073015;%%
  %21 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Boucenna:2014ela}
\bibitem{Boucenna:2014ela} 
  S.~M.~Boucenna, S.~Morisi and J.~W.~F.~Valle,
  %``Radiative neutrino mass in 3-3-1 scheme,''
  Phys.\ Rev.\ D {\bf 90}, no. 1, 013005 (2014)
  doi:10.1103/PhysRevD.90.013005
  [arXiv:1405.2332 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.013005;%%
  %22 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Boucenna:2014dia}
\bibitem{Boucenna:2014dia} 
  S.~M.~Boucenna, R.~M.~Fonseca, F.~Gonzalez-Canales and J.~W.~F.~Valle,
  %``Small neutrino masses and gauge coupling unification,''
  Phys.\ Rev.\ D {\bf 91}, no. 3, 031702 (2015)
  doi:10.1103/PhysRevD.91.031702
  [arXiv:1411.0566 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.91.031702;%%
  %17 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Phong:2014ofa}
\bibitem{Phong:2014ofa} 
  V.~Q.~Phong, H.~N.~Long, V.~T.~Van and L.~H.~Minh,
  %``Electroweak phase transition in the economical 3-3-1 model,''
  Eur.\ Phys.\ J.\ C {\bf 75}, no. 7, 342 (2015)
  doi:10.1140/epjc/s10052-015-3550-2
  [arXiv:1409.0750 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-015-3550-2;%%
  %7 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Boucenna:2015zwa}
\bibitem{Boucenna:2015zwa} 
  S.~M.~Boucenna, J.~W.~F.~Valle and A.~Vicente,
  %``Predicting charged lepton flavor violation from 3-3-1 gauge symmetry,''
  Phys.\ Rev.\ D {\bf 92}, no. 5, 053001 (2015)
  doi:10.1103/PhysRevD.92.053001
  [arXiv:1502.07546 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.053001;%%
  %15 citations counted in INSPIRE as of 28 Apr 2016



%\cite{DeConto:2015eia}
\bibitem{DeConto:2015eia} 
  G.~De Conto, A.~C.~B.~Machado and V.~Pleitez,
  %``Minimal 3-3-1 model with a spectator sextet,''
  Phys.\ Rev.\ D {\bf 92}, no. 7, 075031 (2015)
  doi:10.1103/PhysRevD.92.075031
  [arXiv:1505.01343 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.075031;%%
  %5 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Correia:2015tra}
\bibitem{Correia:2015tra} 
  F.~C.~Correia and V.~Pleitez,
  %``Neutral meson mixing induced by box diagrams in the 3-3-1 model with heavy leptons,''
  Phys.\ Rev.\ D {\bf 92}, 113006 (2015)
  doi:10.1103/PhysRevD.92.113006
  [arXiv:1508.07319 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.113006;%%
  %3 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Okada:2015bxa}
\bibitem{Okada:2015bxa} 
  H.~Okada, N.~Okada and Y.~Orikasa,
  %``Radiative seesaw mechanism in a minimal 3-3-1 model,''
  Phys.\ Rev.\ D {\bf 93}, no. 7, 073006 (2016)
  doi:10.1103/PhysRevD.93.073006
  [arXiv:1504.01204 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.93.073006;%%
  %19 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Binh:2015cba}
\bibitem{Binh:2015cba} 
  D.~T.~Binh, D.~T.~Huong and H.~N.~Long,
  %``Muon anomalous magnetic moment in the supersymmetric economical 3-3-1 model,''
  Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 148}, 1115 (2015)
  [J.\ Exp.\ Theor.\ Phys.\  {\bf 121}, no. 6, 976 (2015)]
  doi:10.7868/S004445101512007X, 10.1134/S1063776115120109
  [arXiv:1504.03510 [hep-ph]].
  %%CITATION = doi:10.7868/S004445101512007X, 10.1134/S1063776115120109;%%
  %5 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hue:2015fbb}
\bibitem{Hue:2015fbb} 
  L.~T.~Hue, H.~N.~Long, T.~T.~Thuc and T.~Phong Nguyen,
  %``Lepton flavor violating decays of Standard-Model-like Higgs in 3-3-1 model with neutral lepton,''
  Nucl.\ Phys.\ B {\bf 907}, 37 (2016)
  doi:10.1016/j.nuclphysb.2016.03.034
  [arXiv:1512.03266 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2016.03.034;%%
  %8 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Pal:1994ba}
\bibitem{Pal:1994ba} 
  P.~B.~Pal,
  %``The Strong CP question in SU(3)(C) x SU(3)(L) x U(1)(N) models,''
  Phys.\ Rev.\ D {\bf 52}, 1659 (1995)
  doi:10.1103/PhysRevD.52.1659
  [hep-ph/9411406].
  %%CITATION = doi:10.1103/PhysRevD.52.1659;%%
  %80 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2002gg}
\bibitem{Dias:2002gg} 
  A.~G.~Dias, V.~Pleitez and M.~D.~Tonasse,
  %``Naturally light invisible axion in models with large local discrete symmetries,''
  Phys.\ Rev.\ D {\bf 67}, 095008 (2003)
  doi:10.1103/PhysRevD.67.095008
  [hep-ph/0211107].
  %%CITATION = doi:10.1103/PhysRevD.67.095008;%%
  %33 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2003zt}
\bibitem{Dias:2003zt} 
  A.~G.~Dias and V.~Pleitez,
  %``Stabilizing the invisible axion in 3-3-1 models,''
  Phys.\ Rev.\ D {\bf 69}, 077702 (2004)
  doi:10.1103/PhysRevD.69.077702
  [hep-ph/0308037].
  %%CITATION = doi:10.1103/PhysRevD.69.077702;%%
  %35 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dias:2003iq}
\bibitem{Dias:2003iq} 
  A.~G.~Dias, C.~A.~de S. Pires and P.~S.~R.~da Silva,
  %``Discrete symmetries, invisible axion and lepton number symmetry in an economic 3 3 1 model,''
  Phys.\ Rev.\ D {\bf 68}, 115009 (2003)
  doi:10.1103/PhysRevD.68.115009
  [hep-ph/0309058].
  %%CITATION = doi:10.1103/PhysRevD.68.115009;%%
  %36 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Mizukoshi:2010ky}
\bibitem{Mizukoshi:2010ky} 
  J.~K.~Mizukoshi, C.~A.~de S.Pires, F.~S.~Queiroz and P.~S.~Rodrigues da Silva,
  %``WIMPs in a 3-3-1 model with heavy Sterile neutrinos,''
  Phys.\ Rev.\ D {\bf 83}, 065024 (2011)
  doi:10.1103/PhysRevD.83.065024
  [arXiv:1010.4097 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.83.065024;%%
  %44 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Boucenna:2015pav}
\bibitem{Boucenna:2015pav} 
  S.~M.~Boucenna, S.~Morisi and A.~Vicente,
  %``The LHC diphoton resonance from gauge symmetry,''
  arXiv:1512.06878 [hep-ph].
  %%CITATION = ARXIV:1512.06878;%%
  %101 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Hernandez:2015ywg}
\bibitem{Hernandez:2015ywg} 
  A.~E.~C.~Hernández and I.~Nisandzic,
  %``LHC diphoton 750 GeV resonance as an indication of $SU(3)_c\times SU(3)_L\times U(1)_X$ gauge symmetry,''
  arXiv:1512.07165 [hep-ph].
  %%CITATION = ARXIV:1512.07165;%%
  %101 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Dong:2015dxw}
\bibitem{Dong:2015dxw} 
  P.~V.~Dong and N.~T.~K.~Ngan,
  %``Phenomenology of the simple 3-3-1 model with inert scalars,''
  arXiv:1512.09073 [hep-ph].
  %%CITATION = ARXIV:1512.09073;%%
  %21 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Cao:2015scs}
\bibitem{Cao:2015scs} 
  Q.~H.~Cao, Y.~Liu, K.~P.~Xie, B.~Yan and D.~M.~Zhang,
  %``Diphoton excess, low energy theorem, and the 331 model,''
  Phys.\ Rev.\ D {\bf 93}, no. 7, 075030 (2016)
  doi:10.1103/PhysRevD.93.075030
  [arXiv:1512.08441 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.93.075030;%%
  %72 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Cao:2015lia}
\bibitem{Cao:2015lia} 
  Q.~H.~Cao, B.~Yan and D.~M.~Zhang,
  %``Simple non-Abelian extensions of the standard model gauge group and the diboson excesses at the LHC,''
  Phys.\ Rev.\ D {\bf 92}, no. 9, 095025 (2015)
  doi:10.1103/PhysRevD.92.095025
  [arXiv:1507.00268 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.095025;%%
  %59 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Grimus:2000vj}
\bibitem{Grimus:2000vj} 
  W.~Grimus and L.~Lavoura,
  %``The Seesaw mechanism at arbitrary order: Disentangling the small scale from the large scale,''
  JHEP {\bf 0011}, 042 (2000)
  doi:10.1088/1126-6708/2000/11/042
  [hep-ph/0008179].
  %%CITATION = doi:10.1088/1126-6708/2000/11/042;%%
  %69 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Alessandria:2011rc}
\bibitem{Alessandria:2011rc} 
  F.~Alessandria {\it et al.},
  %``Sensitivity of CUORE to Neutrinoless Double-Beta Decay,''
  arXiv:1109.0494 [nucl-ex].
  %%CITATION = ARXIV:1109.0494;%%
  %61 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Auger:2012ar}
\bibitem{Auger:2012ar} 
  M.~Auger {\it et al.} [EXO-200 Collaboration],
  %``Search for Neutrinoless Double-Beta Decay in $^{136}$Xe with EXO-200,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 032505 (2012)
  doi:10.1103/PhysRevLett.109.032505
  [arXiv:1205.5608 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.109.032505;%%
  %347 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Abt:2004yk}
\bibitem{Abt:2004yk} 
  I.~Abt {\it et al.},
  %``A New $Ge^{76}$ Double Beta Decay Experiment at LNGS: Letter of Intent,''
  hep-ex/0404039.
  %%CITATION = HEP-EX/0404039;%%
  %223 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Ackermann:2012xja}
\bibitem{Ackermann:2012xja} 
  K.~H.~Ackermann {\it et al.} [GERDA Collaboration],
  %``The GERDA experiment for the search of $0\nu\beta\beta$  decay in $^{76}$Ge,''
  Eur.\ Phys.\ J.\ C {\bf 73}, no. 3, 2330 (2013)
  doi:10.1140/epjc/s10052-013-2330-0
  [arXiv:1212.4067 [physics.ins-det]].
  %%CITATION = doi:10.1140/epjc/s10052-013-2330-0;%%
  %109 citations counted in INSPIRE as of 28 Apr 2016



%\cite{KamLANDZen:2012aa}
\bibitem{KamLANDZen:2012aa} 
  A.~Gando {\it et al.} [KamLAND-Zen Collaboration],
  %``Measurement of the double-\beta decay half-life of ^{136}Xe with the KamLAND-Zen experiment,''
  Phys.\ Rev.\ C {\bf 85}, 045504 (2012)
  doi:10.1103/PhysRevC.85.045504
  [arXiv:1201.4664 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevC.85.045504;%%
  %161 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Albert:2014fya}
\bibitem{Albert:2014fya} 
  J.~B.~Albert {\it et al.} [EXO-200 Collaboration],
  %``Search for Majoron-emitting modes of double-beta decay of $^{136}$Xe with EXO-200,''
  Phys.\ Rev.\ D {\bf 90}, no. 9, 092004 (2014)
  doi:10.1103/PhysRevD.90.092004
  [arXiv:1409.6829 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.90.092004;%%
  %16 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Guiseppe:2011me}
\bibitem{Guiseppe:2011me} 
  C.~E.~Aalseth {\it et al.} [Majorana Collaboration],
  %``The Majorana Experiment,''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 217}, 44 (2011)
  doi:10.1016/j.nuclphysbps.2011.04.063
  [arXiv:1101.0119 [nucl-ex]].
  %%CITATION = doi:10.1016/j.nuclphysbps.2011.04.063;%%
  %24 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Bilenky:2014uka}
\bibitem{Bilenky:2014uka} 
  S.~M.~Bilenky and C.~Giunti,
  %``Neutrinoless Double-Beta Decay: a Probe of Physics Beyond the Standard Model,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 30}, no. 04n05, 1530001 (2015)
  doi:10.1142/S0217751X1530001X
  [arXiv:1411.4791 [hep-ph]].
  %%CITATION = doi:10.1142/S0217751X1530001X;%%
  %51 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Bora:2012tx}
\bibitem{Bora:2012tx} 
  K.~Bora,
  %``Updated values of running quark and lepton masses at GUT scale in SM, 2HDM and MSSM,''
  Horizon {\bf 2} (2013)
  [arXiv:1206.5909 [hep-ph]].
  %%CITATION = ARXIV:1206.5909;%%
  %22 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Xing:2007fb}
\bibitem{Xing:2007fb} 
  Z.~z.~Xing, H.~Zhang and S.~Zhou,
  %``Updated Values of Running Quark and Lepton Masses,''
  Phys.\ Rev.\ D {\bf 77}, 113016 (2008)
  doi:10.1103/PhysRevD.77.113016
  [arXiv:0712.1419 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.77.113016;%%
  %271 citations counted in INSPIRE as of 28 Apr 2016



%\cite{Agashe:2014kda}
\bibitem{Agashe:2014kda} 
  K.~A.~Olive {\it et al.} [Particle Data Group Collaboration],
  %``Review of Particle Physics,''
  Chin.\ Phys.\ C {\bf 38}, 090001 (2014).
  doi:10.1088/1674-1137/38/9/090001
  %%CITATION = doi:10.1088/1674-1137/38/9/090001;%%
  %3666 citations counted in INSPIRE as of 28 Apr 2016




